Multi-tenant Pub/Sub Processing for Real-time Data Streams

Devices and sensors generate streams of data across a diversity of locations and protocols. That data usually reaches a central platform that is used to store and process the streams. Processing can be done in real time, with transformations and enrichment happening on-the-fly, but it can also happen after data is stored and organized in repositories. In the former case, stream processing technologies are required to operate on the data; in the latter batch analytics and queries are of common use. This paper introduces a runtime to dynamically construct data stream processing topologies based on user-supplied code. These dynamic topologies are built on-the-fly using a data subscription model defined by the applications that consume data. Each user-defined processing unit is called a Service Object. Every Service Object consumes input data streams and may produce output streams that others can consume. The subscription-based programing model enables multiple users to deploy their own data-processing services. The runtime does the dynamic forwarding of data and execution of Service Objects from different users. Data streams can originate in real-world devices or they can be the outputs of Service Objects.

==> api.tex <==
\section{REST API}
\label{sec:api}

Service Objects are exposed through a RESTful API that uses HTTP as a transport
and that acts as the SO front-end. This basically implies that SOs can be
identified unambiguously using uniques URIs. The API provides resource
actuations through the four main HTTP operations: GET (retrieve), POST (create),
PUT (update) and DELETE. Table \ref{tab:api} summarizes the COMPOSE Service
Objects API. In the table, soId represents the unique ID associated to each
Service Object registered in the platform.

\begin{table*}
\begin{center}
\begin{tabular}{ | l | l | l | }
\hline
  \centering \textbf{operation} & \centering \textit{\textbf{Target URI}} &
  \multicolumn{1}{|c|}{\textit{\textbf{Role}}} \\  \hline

  Create   & POST \url{/}    & Create a new SO posting a JSON document. \\
  \hline Retrieve & GET \url{/} & Retrieve the list of all the SOs created.\\
  \hline Retrieve & GET \url{/<soId>}         & Retrieve attributes from the
  \texttt{<SO\_Id>} Service Object. \\ \hline Update   & PUT \url{/<soId>}      
  & Modify the \texttt{<SO\_Id>} ServiceObject. \\ \hline Delete   & DEL \url{/<soId>}         & Delete the \texttt{<SO\_Id>} Service Object. \\ 
  \hline Retrieve & GET \url{/<soId>/streams} & Retrieve the list of all the
  SO streams. \\
  \hline Create   & POST \url{/<soId>/streams/<streamId>/subscriptions} &
  Subscribe the Service Object \texttt{<soId>} to a service . \\ \hline Update   &
  PUT \url{/<soId>/streams/<streamId>} & Store \texttt{<soId>} data
  puting a JSON document. \\ \hline Retrieve &
  GET \url{/<soId>/streams/<streamId>} & Retrieve the list of all the data of
  \texttt{<soId>} Service Object. \\
  \hline 
\end{tabular}
\end{center}
\caption{API operations}
\label{tab:api}
\end{table*}



SOs are created by POSTing a JSON document to the \url{/} resource.
The document is a basic description of the main properties of the Service Object
about to be created. The following example illustrates the case of a SmartPhone
object enabled with three different sensors (GPS location, Microphone and
Temperature Sensor), each one becoming a stream of data in the SO abstraction.
The device is also presenting the capability to be activated through the platform:
when the {\it vibrate action} is invoked on it, the device will vibrate to
notify something to the user carrying it. Note that some other fields exist in
the complete version of the Service Object description, but it have been
shortened in this example for the sake of clarity.



\begin{Code}[caption=Creating a Service Object, label=text:create_so]
POST /
Accept: application/json
Content-type: application/json

{ "name":"user21",
  "description":"Smartphone of user21 in deployment",
  "streams": [
      { "name":"location",
        "channels": [ {"name":"lat"}, {"name":"lon"} ],
        "description":"Outdoor location of the smartphone"
      },
      { "name":"microphone",
        "channels": [ {"name":"noise"} ],
        "description":"Quantity of noise"
      },
      { "name":"temperature",
        "channels": [ {"name":"temp"} ],
        "description":"Phone temperature"
      }
    ],
  "actions":["vibrate"]
}
\end{Code}



The corresponding response message contains the field \texttt{"id"} that is the
unique identifier of the SO within the COMPOSE platform (the \texttt{<soId>} specified in Table
\ref{tab:api}). The response also contains the list of the \texttt{<streamsId>}
in the field \texttt{"streams"}. 

\begin{Code}[caption=Retrieving the Service Object description,
label=text:get_so] 
{ "id": "13740600949717e0426e5fdf34e6998aa00b865",
  "name": "user21",
  "createdAt": 1379402251644,
  "updatedAt": 1379402251644,
  "description": "Smartphone of user21 in deployment",
  "streams": ["location", "microphone", "temperature"],
  "actions": ["vibrate"]
}
\end{Code}


Requesting the list of all the \texttt{<soId>}
streams 
% would be requested through the following URL:
% {\small
% \begin{verbatim}
% /13740600949717e0426e5fdf34e6998aa00b865/
% \end{verbatim}
% }
% 
% And 
would result in the following JSON document as a response for the
particular example of the SmartPhone.

\begin{Code}[caption=Retrieving the Streams of a Service Object,
label=text:get_so_streams] 
{ "streams": [
    { "name": "location",
      "channels": ["lat", "lon"],
      "description": "The location of the samartphone."
    },
    { "name": "microphone",
      "channels": ["noise"],
      "description": "Quantity of noise"
    },
    { "name": "temperature",
      "channels": ["temp"],
      "description": "Phone temperature",
    } ]
}
\end{Code}


% Retrieve all the SOs (\url{/}) results in an array of all the \texttt{<soId>}s stored.
% 
% {\small
% \begin{verbatim}
% ["13740600949717e0426e5fdf34e6998aa00b865", ... , 
% "34q34234q34ed345qw3434"]
% \end{verbatim}
% }



As discussed in Section~\ref{sec:serviceobjects} a SO update is actually a JSON
document containing, among other information, a tuple of values that correspond
to the channels of a device sensor, what is represented as a {\it stream} in
the SO representation. 

An example of pushing data from the SmartPhone to
its corresponding SO counter-part is achieved by submitting the following JSON
data in the body request for the \url{/<soId>/streams/<streamId>/store.data}
url. The \texttt{<soId>} would be obtained from the previous creation of the
SO. \texttt{streamId} should be picked from the list of streams existing in the
SO description. In this example, temperature data is being pushed to the
platform. As it can be observed in the following JSON document, the information
for the {\it temp} channel, which is associated to the temperature stream,
includes the actual temperature value as well as other information such as
units, update time and a series of custom fields that the WO can decide to add
when generating the SU for future reference.

\begin{Code}[caption=Posting Data,
label=text:put_so_data] 
{ "channels": [ 
    { "name": "temp",
      "current-value": 22.58,
      "type": "numeric", 
      "unit": "m/s2" 
    } ],
    "name": "temperature",
    "lastUpdate": 194896800, 
    "customFields": {
        "covered-period": "24h",
        "averageLastHour": 32, 
        "risk": "low", 
        "averageLastDay": 42
    }
}
\end{Code}


To retrieve and delete a SO, the corresponding operation can be invoked for
each \texttt{<soId>} URL. For the former a response JSON document describing the
success of the operation is generated, as well as a 200 HTTP status code. For
the latter, a new SO description must be associated to the PUT HTTP operation
on the \texttt{<soId>} URL, resulting in the SO description being updated and a
response generated analogously to the SO creation case described above.

Finally, retrieving  data associated to a SO stream results in a JSON document
containing an array of all the tuples stored for this stream. 

The creation of subscriptions is at the core of the COMPOSE platform and allows
for the definition of data processing paths that are followed by SUs being
generated by external WOs and afterwards ingested by the platform. Subscriptions
can be internal (when one SO wants to get SUs generated by other SOs to be
forwarded to it), or external, when entities outside of the COMPOSE platform
wants to be notified about any SUs produced by one particular SO. 
The following
example illustrates the case of an external URL
(\url{http://external.eu/process}) that wants to be used to forward SUs
generated by the SO with ID <soId>. Note how the subscription document includes the
URL and the HTTP method to be used to forward the data to the external entity.

\begin{Code}[caption=Create a subscription,
label=text:create_so_subscription] 
POST /<soId>/streams/<streamId>/subscriptions HTTP/1.0
Accept: application/json
Content-type: application/json

{
	"type":"http.callback",
	"callbackUrl":"http://external.eu/process"
	"method":"POST"
}
\end{Code}





